Opposing Half Guards

We study the art gallery problem for opposing half guards: guards that can either see to their left or to their right only. We present art gallery theorems, show that the location of half guards in 2-guardable polygons is not restricted to extensions, show that the problem is NP-hard in monotone polygons, and present approximation algorithms for spiral and staircase polygons.

==> Figures/intersect <==
#!/usr/bin/python
#
# 'intersection' takes two line segments (eight coordinates) and computes the intersection point of the segments. 
# 

import sys


def minus(v1,v2): return [v1[0]-v2[0],v1[1]-v2[1]]

def intersection(p1,q1,p2,q2):
    # Find s,t s.t. (1-s)*p1+s*q1 = (1-t)*p2+t*q2
    print p1, q1, p2, q2
    u1 = minus(q1,p1)
    u2 = minus(q2,p2)
    v  = minus(p2,p1)
    print u1, u2, v,
    t  = (v[1]*u1[0]*1.0-v[0]*u1[1]*1.0)/(u2[0]*u1[1]*1.0-u2[1]*u1[0]*1.0)
    print t
    return [p2[0]+t*u2[0],p2[1]+t*u2[1]]

lines = [[[0,0],[0,0]],[[0,0],[0,0]]]
arg = 1
try:
    for segment in range(2):
        for point in range(2):
            for coord in range(2):
                lines[segment][point][coord] = int(sys.argv[arg])
                arg +=1
except: 
    print "Provide two line segments, eight integer coordinates in the format 'x11 y11 x12 y12 x21 y21 x22 y22'!\nExiting program!!!"
    sys.exit(0)

print lines
print "Intersection point is:\n"+str(intersection(lines[0][0],lines[0][1],lines[1][0],lines[1][1]))



==> correctness.tex <==
Let \BB\ be the set of prespecified and computed points on the convex boundary chain of \P\ where the algorithm can place a backward guard. Similarly, let \FF\ be the set of points where the algorithm can place a forward guard. We have $|\BB\cup\FF|\in O(n^2)$. Consider an optimum set of half guards \OPT\ that we can assume by Lemma~\ref{lem:convexboundary} all lie on the convex chain. Follow the convex chain from \u\ to \u'\ until a half guard \ga\ in \OPT\ is reached that does not lie on a point in \BB, if \ga\ is a backward guard, or a point in \FF, if \ga\ is a forward guard. Let \p\ be the last point on the reflex chain seen by the guards in \OPT\ that lie before \ga\ in \OPT. If \ga\ is the first half guard, then $\p=\u$. We will show that we can exchange \ga\ and the subsequent half guard \gb\ in \OPT\ for three half guards \g, \g', and \g''\ that indeed lie on the corresponding points in \BB\ or \FF, respectively. Repeating the argument as the process follows the convex chain in clockwise order, proves our claim.

If \ga\ can be moved to the subsequent point in \BB\ or \FF, depending on its type, without losing visibility, we do so. This will not increase the number of guards.

Assume now that \ga\ is a forward guard in between two subsequent points \q\ and \q'\ in \FF\ and that \ga\ cannot be moved to \q'\ without losing visibility. Assume furthermore that \gb\ is a forward guard.


==> proofs.tex <==
{
\input{mathspiral}
%\section*{Proof of Lemma~\ref{lem:window}}
\begin{proof}[of Lemma~\ref{lem:window}]
Consider the maximal vertical segment $s$ through \p\ in \P. If $s$ does not degenerate into a point (equalling the point \p\ itself), then $s$ is a window of \VP{\p}. Since \P\ has only one reflex boundary chain, \p\ half-sees at most one connected subchain of the reflex boundary chain. Let \r\ and \r'\ be the reflex endpoints of this connected subchain. \VP{\p} has a window collinear to the line segment $[\p,\r]$ issuing from \r\ away from \p\ until it hits the polygon boundary (unless the window degenerates into the point \r) and similarly a window collinear to the line segment $[\p,\r']$ issuing from \r'\ away from \p\ until it hits the polygon boundary (again unless the window degenerates into a point at \r'). No further windows can exist since \P\ has only one reflex boundary chain.
\end{proof}


We denote the windows of \VP{\p} as the $v$-window, the vertical window through \p\, if it exists, and the at most two $r$-windows connecting a reflex vertex and the convex boundary chain of~\P; see Figure~\ref{fig:spiral}(a).%

\begin{proof}[of Lemma~\ref{lem:convexboundary}]
Consider any half-guard set \GG\ and pick a half-guard \g\ from \GG. If \g\ half-sees all of \P, then \g\ must by necessity lie on the convex boundary chain, otherwise \g\ has a $v$-window of non-zero length and the region behind the $v$-window is not seen.

If \g\ does not half-see any points of the reflex boundary chain, then \VP{\g} is a convex region and we can slide \g\ along its $v$-window until it reaches the boundary without losing coverage.
%there is a point on the convex boundary chain from which a half-guard \g'\ (with the opposite visibility orientation) sees the complete convex region. We can therefore replace \g\ by \g'\ in~\Gg.

If \g\ half-sees points of the reflex boundary, consider the maximal subchain \CC{\g} of the reflex boundary chain that is half-seen by \g. If \CC{\g} is equal to the complete reflex boundary chain, then \g\ half-sees both \u\ and \u'\ and we can let \g\ slide along the extension of the segment $[\u,\g]$ away from \u\ until it hits the convex boundary without losing coverage. If \CC{\g} does not half-see the complete reflex boundary chain, then assume without loss of generality that \u\ is not half-seen by \g. If \u\ is seen, we use \u'\ instead in the following argument. Walk from \u\ along the reflex boundary chain until the first reflex vertex that is half-seen by \g. Denote this vertex \v. Vertex \v\ is an endpoint of \CC{\g} and we can let \g\ slide along the extension of the segment $[\v,\g]$ away from \v\ until it hits the convex boundary without losing coverage.

Thus, any half-guard set can be moved so that they all lie on the convex boundary chain while maintaining coverage and the size of the half-guard set.
\end{proof}


\begin{proof}[of Lemma~\ref{lem:threehalves}]
The correctness of the algorithm follows by construction, since it ensures that each window created by a half guard is seen by the next half guard placed.

It remains to show the approximation ratio for the algorithm. To do so, let \BB\ be the set of prespecified and computed points on the convex boundary chain of \P\ where the algorithm can place a backward guard. Similarly, let \FF\ be the set of points where the algorithm can place a forward guard. We have $|\BB\cup\FF|\in O(n^2)$. Consider an optimum set of half guards \OPT\ that we can assume by Lemma~\ref{lem:convexboundary} all lie on the convex chain. Follow the convex chain from \u\ to \u'\ until a half guard \ga\ in \OPT\ is reached that does not lie on a point in \BB, if \ga\ is a backward guard, or a point in \FF, if \ga\ is a forward guard. Let \p\ be the last point on the reflex chain seen by the guards in \OPT\ that lie before \ga\ in \OPT. If \ga\ is the first half guard, then $\p=\u$. We will show that we can exchange \ga\ and the subsequent half guard \gb\ in \OPT\ for three half guards \g, \g', and \g''\ that indeed lie on the corresponding points in \BB\ or \FF, respectively. Repeating the argument as the process follows the convex chain in clockwise order, proves our claim.

If \ga\ can be moved to the subsequent point in \BB\ or \FF, depending on its type, without losing visibility, we do so. This will not increase the number of guards.

Assume that \ga\ is a backward guard between two subsequent points \q\ and \q'\ in \BB\ and that \ga\ cannot be moved to \q'\ without losing visibility. Let $v_{i-1}$ be the first vertex on the reflex chain that \ga\ sees and thus \ga\ sees $e_i$. So, \p\ is some point on $e_i$ (not $v_{i}$). Since \ga\ cannot be moved to \q'\ and the reflex chain is seen by the previous guards until \p\ on $e_i$, there must be points on the convex chain that are not seen if \ga\ is moved towards \q'. Let \r\ be such a point on the convex chain and let \gz\ be the guard in \OPT\ that sees \r. The guard \gz\ must be a backward guard at \r\ and \r\ is by assumption in \BB, hence, \ga\ can be moved to the intersection of the supporting line from \r\ through the reflex chain and the convex chain. But this point lies in \BB, a contradiction. 

Assume now that \ga\ is a forward guard between two subsequent points \q\ and \q'\ in \FF\ and that \ga\ cannot be moved to \q'\ without losing visibility. Let $v_i$ be the last vertex on the reflex chain that \ga\ sees and assume furthermore that \gb\ is a forward guard. Without loss of generality, we can assume that \gb\ lies on \spp{\ga}\ or on \tp{v_i}, whichever is closer to \ga. If \gb\ does not we can move it there without losing visibility.
%
We can place two forward guards \g\ and \g'\ at \q\ and \q'. The half guard \g'\ sees a vertex $v_{i'}$ with $i\leq i'$, hence we can replace \gb\ by a half guard at \spp{\q'}\ or at \tp{v_{i'}}, if $v_{i'}$ is an inner corner. In any case, \ga\ and \gb\ are replaced with three guards at positions in~\FF.

Finally, assume that \ga\ is a forward guard and that the subsequent guard \gb\ in \OPT\ is backward. We can argue for \gb\ as we did in the first case to obtain a point \r\ on the convex chain not seen by \gb\ if \gb\ is moved forward. The forward guard \ga\ lies on the intersection between vertical line segment intersection through \r\ and the convex chain (the vertical segment spans between \r\ and \ga). Thus, the convex region defined by the convex chain from \r\ to \ga\ and limited by the vertical segment through these points is seen by \gb\ and it contains a corner.
%
We can replace \ga\ and \gb\ by a half guard \g\ at the corner, a forward guard \g'\ at \tp{v_i}, where $v_i$ is the last reflex vertex seen be \g, and either a backward guard at \ext{e_{i'}}, where $e_{i'}$ is the first unseen edge of the reflex boundary, or a half guard at the subsequent corner, whichever point comes first along a traversal of the convex chain.

In each case, a pair of half guards from the optimum is replaced by a triple of half guards at a subset of our designated positions. Hence, there exists a feasible placement of half guards having size at most $\lceil3|\OPT|/2\rceil$. Since the dynamic programming algorithm computes the minimum such placement, the lemma follows.
\end{proof}

%If \ga\ lies after \tp{\pa}\ and is a backward guard, then the algorithm can choose to place $\g=\ext{e_i}$ and then independently of whether \gb\ is forward or backward guard, the algorithm can choose to place \g'\ 
%\end{proof}


}
